MuRAR: A Simple and Effective Multimodal Retrieval and Answer Refinement Framework for Multimodal Question Answering

Recent advancements in retrieval-augmented generation (RAG) have demonstrated impressive performance in the question-answering (QA) task. However, most previous works predominantly focus on text-based answers. While some studies address multimodal data, they still fall short in generating comprehensive multimodal answers, particularly for explaining concepts or providing step-by-step tutorials on how to accomplish specific goals. This capability is especially valuable for applications such as enterprise chatbots and settings such as customer service and educational systems, where the answers are sourced from multimodal data. In this paper, we introduce a simple and effective framework named MuRAR (Multimodal Retrieval and Answer Refinement). MuRAR enhances text-based answers by retrieving relevant multimodal data and refining the responses to create coherent multimodal answers. This framework can be easily extended to support multimodal answers in enterprise chatbots with minimal modifications. Human evaluation results indicate that multimodal answers generated by MuRAR are more useful and readable compared to plain text answers.

==> backup_materials.tex <==
\subsection{Human Evaluation Statistic Results}

--------------------------------------------------------------------------------------------------
-------------------------------------------------
Annotator No.0 has 294 answers.
	Their average usefulness score: 3.6462585034013606, average readability score: 3.836734693877551, average relevance score: 4.017006802721088.
	Their preference: 207 (70.40816326530613%) Multi-Modal, 41 (13.945578231292515%) Text Only 46 (15.646258503401361%) Same
-------------------------------------------------
Annotator No.1 has 237 answers.
	Their average usefulness score: 2.8860759493670884, average readability score: 3.029535864978903, average relevance score: 3.270042194092827.
	Their preference: 115 (48.52320675105485%) Multi-Modal, 81 (34.177215189873415%) Text Only 41 (17.29957805907173%) Same
-------------------------------------------------
Annotator No.2 has 259 answers.
	Their average usefulness score: 3.7451737451737452, average readability score: 3.833976833976834, average relevance score: 3.8764478764478763.
	Their preference: 205 (79.15057915057915%) Multi-Modal, 28 (10.81081081081081%) Text Only 26 (10.038610038610038%) Same
-------------------------------------------------
Annotator No.3 has 53 answers.
	Their average usefulness score: 3.056603773584906, average readability score: 3.509433962264151, average relevance score: 3.5849056603773586.
	Their preference: 30 (56.60377358490566%) Multi-Modal, 16 (30.18867924528302%) Text Only 7 (13.20754716981132%) Same
-------------------------------------------------
Annotator No.4 has 9 answers.
	Their average usefulness score: 4.111111111111111, average readability score: 4.444444444444445, average relevance score: 4.444444444444445.
	Their preference: 9 (100.0%) Multi-Modal, 0 (0.0%) Text Only 0 (0.0%) Same
-------------------------------------------------
Annotator No.5 has 22 answers.
	Their average usefulness score: 4.0, average readability score: 4.090909090909091, average relevance score: 4.181818181818182.
	Their preference: 19 (86.36363636363636%) Multi-Modal, 2 (9.090909090909092%) Text Only 1 (4.545454545454546%) Same
-------------------------------------------------
Annotator No.6 has 24 answers.
	Their average usefulness score: 4.25, average readability score: 4.208333333333333, average relevance score: 4.625.
	Their preference: 23 (95.83333333333334%) Multi-Modal, 0 (0.0%) Text Only 0 (0.0%) Same
-------------------------------------------------
Annotator No.7 has 2 answers.
	Their average usefulness score: 4.0, average readability score: 4.5, average relevance score: 4.5.
	Their preference: 2 (100.0%) Multi-Modal, 0 (0.0%) Text Only 0 (0.0%) Same
--------------------------------------------------------------------------------------------------
-------------------------------------------------
The average usefulness score for GPT3.5 among three annotators is 3.34
The average usefulness score for GPT4 among three annotators is 3.6
The average usefulness score for both GPT among three annotators is 3.47
The average readability score for GPT3.5 among three annotators is 3.493333333333333
The average readability score for GPT4 among three annotators is 3.7622222222222224
The average readability score for both GPT among three annotators is 3.6277777777777773
The average relevance score for GPT3.5 among three annotators is 3.6644444444444444
The average relevance score for GPT4 among three annotators is 3.8955555555555557
The average relevance score for both GPT among three annotators is 3.78
-------------------------------------------------
The preference rate for GPT3.5 is 0.82
The preference rate for GPT4 is 0.9
The preference rate for both GPT is 0.86
-------------------------------------------------
The standard deviation for usefulness scores for GPT3.5 is 0.9740864666160004
The standard deviation for usefulness scores for GPT4 is 0.9059474271395337
The standard deviation for usefulness scores is 0.9495749536464158
The standard deviation for readability scores for GPT3.5 is 0.768567691421059
The standard deviation for readability scores for GPT4 is 0.7058870612285485
The standard deviation for readability scores is 0.7500411511344306
The standard deviation for relevance scores for GPT3.5 is 0.8576424763757627
The standard deviation for relevance scores for GPT4 is 0.8301152679144574
The standard deviation for relevance scores is 0.851865056258369
-------------------------------------------------
Results for None modification (Normal)
The overall krippendorff alpha is 0.4179276400904499
The overall cohen kappa is 0.16311660049114965
The krippendorff alpha for usefulness scores for GPT3.5 is 0.41498093145786374
The cohen kappa for usefulness scores for GPT3.5 is 0.14926378757021755
The krippendorff alpha for usefulness scores for GPT4 is 0.5423725981620717
The cohen kappa for usefulness scores for GPT4 is 0.24079546796471074
The krippendorff alpha for usefulness scores is 0.4758232142364366
The cohen kappa for usefulness scores is 0.19488674351857907
The krippendorff alpha for readability scores for GPT3.5 is 0.34179639933307104
The cohen kappa for readability scores for GPT3.5 is 0.09691324886475557
The krippendorff alpha for readability scores for GPT4 is 0.3187455791275424
The cohen kappa for readability scores for GPT4 is 0.13000494659499287
The krippendorff alpha for readability scores is 0.3424178801219099
The cohen kappa for readability scores is 0.11501641482330445
The krippendorff alpha for relevance scores for GPT3.5 is 0.3368642245811351
The cohen kappa for relevance scores for GPT3.5 is 0.13277131893444563
The krippendorff alpha for relevance scores for GPT4 is 0.4464575214165398
The cohen kappa for relevance scores for GPT4 is 0.19246877284539587
The krippendorff alpha for relevance scores is 0.39254053222954577
The cohen kappa for relevance scores is 0.16337621550515632
-------------------------------------------------
Results for combined 2-3 and 4-5 (Merging)
The overall krippendorff alpha is 0.3437493356670611
The overall cohen kappa is 0.3154045276625094
The krippendorff alpha for usefulness scores for GPT3.5 is 0.3468140820482979
The cohen kappa for usefulness scores for GPT3.5 is 0.3178533217936328
The krippendorff alpha for usefulness scores for GPT4 is 0.4993176219958725
The cohen kappa for usefulness scores for GPT4 is 0.4378312135241001
The krippendorff alpha for usefulness scores is 0.4163502277345903
The cohen kappa for usefulness scores is 0.376537859338502
The krippendorff alpha for readability scores for GPT3.5 is 0.2146605183653999
The cohen kappa for readability scores for GPT3.5 is 0.16760781476709116
The krippendorff alpha for readability scores for GPT4 is 0.25024667931688793
The cohen kappa for readability scores for GPT4 is 0.27811578884431115
The krippendorff alpha for readability scores is 0.23741330272940464
The cohen kappa for readability scores is 0.22275876029596112
The krippendorff alpha for relevance scores for GPT3.5 is 0.2958229813664597
The cohen kappa for relevance scores for GPT3.5 is 0.29768602763939195
The krippendorff alpha for relevance scores for GPT4 is 0.36638988874345546
The cohen kappa for relevance scores for GPT4 is 0.36056390710340397
The krippendorff alpha for relevance scores is 0.33231686005871663
The cohen kappa for relevance scores is 0.329914839548697
-------------------------------------------------
Results for drop\_outliers
The overall krippendorff alpha is 0.9023314552544957
The overall cohen kappa is 0.7100491137872653
The krippendorff alpha for usefulness scores for GPT3.5 is 0.9167414374555243
The cohen kappa for usefulness smcores for GPT3.5 is 0.6878793133344894
The krippendorff alpha for usefulness scores for GPT4 is 0.9263475811547482
The cohen kappa for usefulness scores for GPT4 is 0.7900182592818016
The krippendorff alpha for usefulness scores is 0.9217896258002837
The cohen kappa for usefulness scores is 0.7382740876560004
The krippendorff alpha for readability scores for GPT3.5 is 0.8859760947493436
The cohen kappa for readability scores for GPT3.5 is 0.6851574212893553
The krippendorff alpha for readability scores for GPT4 is 0.8814266160084943
The cohen kappa for readability scores for GPT4 is 0.7047619047619047
The krippendorff alpha for readability scores is 0.8860547158717532
The cohen kappa for readability scores is 0.6968165740272865
The krippendorff alpha for relevance scores for GPT3.5 is 0.881174066083797
The cohen kappa for relevance scores for GPT3.5 is 0.6459266432635274
The krippendorff alpha for relevance scores for GPT4 is 0.8967897825336555
The cohen kappa for relevance scores for GPT4 is 0.7291196388261851
The krippendorff alpha for relevance scores is 0.8894764033570917
The cohen kappa for relevance scores is 0.6871741397288842



% EMNLP 2024 review
1. Clarify Technical and Design Details:
Issue: Reviewers pointed out that some technical aspects, especially the encoding of multimodal data, are unclear.
Improvement: Add more operational and technical design details, including how multimodal data is encoded and how it integrates into the QA framework. Ensure the steps are sufficiently detailed to allow other researchers to understand and implement method. This will also help address concerns about flexibility and reproducibility.
2. Increase Transparency on Data and Baselines (Reviewer 3, Reviewer 2)
Issue: Reviewers mentioned the limited sample size (~300), the absence of baselines for comparison, and the lack of public access to the code or dataset.
Improvement: Consider releasing part of the dataset or code to enhance transparency. Additionally, include comparisons with other state-of-the-art multimodal QA systems or establish a baseline (e.g., text-based RAG) to show MuRAR’s relative performance improvements.
3. Address Reproducibility Concerns
Issue: Multiple reviewers highlighted challenges in reproducing results due to limited dataset size and vague technical details.
Improvement: Provide more clarity on experimental settings and conditions. Specify tools, algorithms, or datasets used to reduce variance in reproducibility attempts. Clearly explain any limitations or restrictions caused by using proprietary systems (e.g., GPT).
4. Enhance Multimodal Retrieval Explanation
Issue: There are questions about whether the multimodal retrieval process can handle long or noisy queries effectively.
Improvement: Address how MuRAR deals with these scenarios in your paper. Explain any strategies used to manage long queries, potential errors, or noise, and clarify how the system prioritizes or refines relevant multimodal content.
5. Incorporate Ethical and Privacy Considerations
Issue: The reliance on closed-source models (e.g., GPT) was flagged as problematic due to potential privacy concerns.
Improvement: Include a discussion of the ethical implications and privacy issues related to using closed-source systems. Consider offering suggestions for mitigating these risks, such as alternative approaches or data privacy protocols.
6. Add Source Attribution for Visual Content
Issue: Reviewer 1 suggested that providing the source or URL for visual content (e.g., images or diagrams) in the answers could improve user experience.
Improvement: Consider adding this feature to MuRAR and mention it in the paper, as it could enhance the system’s transparency and usability for end users.


